Enabling Collaborative Clinical Diagnosis of Infectious Keratitis by Integrating Expert Knowledge and Interpretable Data-driven Intelligence

Although data-driven artificial intelligence (AI) in medical image diagnosis has shown impressive performance in silico, the lack of interpretability makes it difficult to incorporate the "black box" into clinicians' workflows. To make the diagnostic patterns learned from data understandable by clinicians, we develop an interpretable model, knowledge-guided diagnosis model (KGDM), that provides a visualized reasoning process containing AI-based biomarkers and retrieved cases that with the same diagnostic patterns. It embraces clinicians' prompts into the interpreted reasoning through human-AI interaction, leading to potentially enhanced safety and more accurate predictions. This study investigates the performance, interpretability, and clinical utility of KGDM in the diagnosis of infectious keratitis (IK), which is the leading cause of corneal blindness. The classification performance of KGDM is evaluated on a prospective validation dataset, an external testing dataset, and an publicly available testing dataset. The diagnostic odds ratios (DOR) of the interpreted AI-based biomarkers are effective, ranging from 3.011 to 35.233 and exhibit consistent diagnostic patterns with clinic experience. Moreover, a human-AI collaborative diagnosis test is conducted and the participants with collaboration achieved a performance exceeding that of both humans and AI. By synergistically integrating interpretability and interaction, this study facilitates the convergence of clinicians' expertise and data-driven intelligence. The promotion of inexperienced ophthalmologists with the aid of AI-based biomarkers, as well as increased AI prediction by intervention from experienced ones, demonstrate a promising diagnostic paradigm for infectious keratitis using KGDM, which holds the potential for extension to other diseases where experienced medical practitioners are limited and the safety of AI is concerned.

==> figures/dor_table.tex <==


\begin{tabular}{llrlr}
\toprule
name &       disease &  odd\_ratio &              CI95 &  pvalue \\
\midrule
  P0 &        Amoeba &      28.60 & (24.0708-33.9741) &    0.00 \\
  P1 &        Amoeba &      21.01 & (12.4466-35.4559) &    0.00 \\
  P2 &        Amoeba &      43.51 & (37.7746-50.1081) &    0.00 \\
  P4 &        Amoeba &      25.96 & (21.1432-31.8793) &    0.00 \\
  P7 &        Amoeba &      17.34 & (15.0962-19.9233) &    0.00 \\
  P8 &        Amoeba &      48.11 & (41.7572-55.4349) &    0.00 \\
 P11 &          Bact &       5.52 &  (0.5001-60.9029) &    0.23 \\
 P15 &          Bact &       5.55 &  (2.4867-12.3699) &    0.00 \\
 P19 &          Bact &       5.40 &   (3.9548-7.3619) &    0.00 \\
 P22 &        Fungal &       7.27 &   (6.4480-8.1864) &    0.00 \\
 P28 &        Fungal &      13.40 & (11.6998-15.3558) &    0.00 \\
 P31 &           Hsk &       7.80 &   (6.3628-9.5732) &    0.00 \\
 P33 &           Hsk &       7.97 &   (6.4965-9.7737) &    0.00 \\
 P35 &           Hsk &       7.33 &   (5.9756-8.9924) &    0.00 \\
 P39 &           Hsk &       7.93 &   (6.4687-9.7320) &    0.00 \\
\bottomrule
\end{tabular}

